Variational Multiscale Evolve and Filter Strategies for Convection-Dominated Flows

The evolve-filter (EF) model is a filter-based numerical stabilization for under-resolved convection-dominated flows. EF is a simple, modular, and effective strategy for both full-order models (FOMs) and reduced-order models (ROMs). It is well-known, however, that when the filter radius is too large, EF can be overdiffusive and yield inaccurate results. To alleviate this, EF is usually supplemented with a relaxation step. The relaxation parameter, however, is very sensitive with respect to the model parameters. In this paper, we propose a novel strategy to alleviate the EF overdiffusivity for a large filter radius. Specifically, we leverage the variational multiscale (VMS) framework to separate the large resolved scales from the small resolved scales in the evolved velocity, and we use the filtered small scales to correct the large scales. Furthermore, in the new VMS-EF strategy, we use two different ways to decompose the evolved velocity: the VMS Evolve-Filter-Filter-Correct (VMS-EFFC) and the VMS Evolve-Postprocess-Filter-Correct (VMS-EPFC) algorithms. The new VMS-based algorithms yield significantly more accurate results than the standard EF in both the FOM and the ROM simulations of a flow past a cylinder at Reynolds number Re = 1000.

==> sections/VMSSM.tex <==
\section{Variational multi-scale Smagorinsky}
\label{sec:VMS-SM}
This section describes a VMS-Smagorinsky model. In this approach, the Eddy-viscosity is only applied to the small resolved scales.
\subsection{The Model} We present the unsteady Smagorinsky model. The model is defined at the discrete level, however, for the sake of presentation, we treat it as a continuous model to clarify its bound with Navier-Stokes equations.\\
Let us consider a spatial domain $\Omega \subset \mathbb R^d$, for $d = 1,2,3$, with Lipschitz-continuous boundary $\partial \Omega$. The boundary is such that $\partial \Omega = \Gamma_N \cup \Gamma_D$ and $\Gamma_N \cap \Gamma_D = \emptyset $ with $\Gamma_N$ and $\Gamma_D$ featuring ``free-flow" boundary conditions and Dirichlet boundary conditions, respectively.
The goal is to approximate the velocity $u(x, t) \doteq u: {\Omega}  \mapsto {\mathbb R^2}$ and pressure $p(x, t) \doteq  p : \Omega \mapsto  \mathbb R$ solving, for $t \in (0,T)$:
 \begin{equation}
\label{eq:NSE}
\begin{cases}
 \displaystyle u_t  - \nabla \cdot (\nu \nabla u + \nu_T(u')\nabla u' ) + (u \cdot \nabla) u + \nabla p = 0 & \text{in }  \Omega \times (0, T), \\
\nabla \cdot u = 0  & \text{in }  \Omega \times (0, T), \\
u = u_D & \text{on } \Gamma_D \times (0, T), \\
\displaystyle -p n + \nu \frac{{\partial} u}{\partial n} + \nu_T(u') \frac{{\partial} u'}{\partial n}  = 0  & \text{on }  \Gamma_N \times (0, T), \\
u(x, 0) = u_0 & \text{in }  \Omega,
\end{cases}
\end{equation}
where $u'$ denotes the resolved small-scales of $u$, $u_0$ is an initial condition, $u_D$ is a given Dirichlet boundary condition, $\nu$ is the kinematic viscosity and $\nu_T(u')$ is the Eddy viscosity (we postpone the specific definition of the Eddy viscosity in the next section). \\
We now define the velocity space $\mathbb U = \{u \in [H^1(\Omega)]^d \; \text{s.t.}\ u_{|_{\Gamma_D}} = 0\}$ and the space $\mathbb Q = L^2(\Omega)$. The problem \eqref{eq:NSE} can be recast in weak formulation as: find $(u,p) \in \mathbb U \times \mathbb Q$ such that
\begin{equation}
\label{eq:NSE}
\begin{cases}
 \displaystyle \int_{\Omega} u_t\cdot v \; dx
	+ a(u,  v)
	+ c(u; u, v)  - b(v, p) + a_s(u;u,v)  = 0 & \forall v \in \mathbb U
	, \\[0.5cm]
b( u,  q ) = 0 & \forall q \in \mathbb Q,
\end{cases}
\end{equation}
where 
 \begin{align*}
    a(u,v) & = \int_{\Omega} \nu \nabla u : \nabla v \; dx, \quad b(v,p)  = \int_{\Omega} p \nabla \cdot v \; dx, \\ 
    c(w;u,v) & = 
    \frac{1}{2}\left (\int_{\Omega} (w \cdot \nabla)u \cdot v\; dx - \int_{\Omega} (w \cdot \nabla)v \cdot u\; dx \right ) \quad \text{and}  & \\
    a_s(u;u,v) & =  \int_{\Omega} \nu_T(u')\nabla u' : \nabla v' \; dx.
    \end{align*}

\subsection{The Discrete Model}
Let us define a uniform regular triangulation $\mathcal T$ over $\Omega$. Its elements are denoted with $K$. We employ the Finite Element (FE) discretization. Defining the space $$\mathbb X^n = \{v \in C^0(\overline{\Omega} \text{ s.t. } v_{|_K} \in \mathbb P_n(K), \; \forall K \in \mathcal T\},$$ where $\mathbb P_n$ is the space of polynomial of degree at most $n$. The FE for velocity and pressure read as $\mathbb U_h \doteq \mathbb U \cap \mathbb X^m$ and $\mathbb Q_h \doteq  \mathbb Q \cap \mathbb X^l$, for $m, l$ positive integers. 
We assume that the two discrete spaces can be decomposed in the following direct sums as \ms{cite book}
\begin{equation}
    \label{eq:decomposition}
    \mathbb U_h = \widetilde{\mathbb U}_h \oplus \mathbb U_h' \quad \text{and} \quad   \mathbb Q_h = \widetilde{\mathbb Q}_h \oplus \mathbb Q_h',
\end{equation}
such that $u_h = \widetilde{u}_h + {u'}_h \in \mathbb U_h$ and
$p_h = \widetilde{p}_h + {p'}_h \in \mathbb Q_h$ present a unique decomposition. Moreover, we define the restriction operator $\Pi_h: \mathbb U_h \rightarrow \widetilde{\mathbb U}_h$ defined as $\Pi_h u_h = \tilde{u}_h$, for all $u_h \in \mathbb U_h$. \\
In this way, setting $\overline{\Pi}_h =(I - \Pi_h)$ the resolved small-scales of the velocity field are approximated as ${u'}_h = (I - \Pi_h)u_h = \overline{\Pi}_h u_h$.
In time, we perform an Implicit Euler scheme with timestep $\Delta t$. A time instance is $t_n = n\Delta t$ for $n = 0, \dots, N_T$ with final time $T = N_T\Delta t$. The solution at time $t^n$ is denoted with $(u^{n}, p^{n})$. The final discrete system reads at time $t^{n+1}$ is: find $(u^{n+1},p^{n+1}) \in \mathbb U_h \times \mathbb Q_h$ such that
\begin{equation}
\label{eq:NSE}
\begin{cases}
 \displaystyle \int_{\Omega} \frac{u^{n+1} - u^{n}}{\Delta t}\cdot v^{n+1}_h \; dx
	+ a(u^{n+1},  v^{n+1})
	+ c(u^{n+1}; u^{n+1}, v^{n+1}) & \\ \quad \quad\quad\quad \quad\quad\quad\quad\quad
 \quad\quad\quad\quad\quad - b(v^{n+1}, p^{n+1}) + a_s(u^{n+1};u^{n+1},v^{n+1})  = 0 & \forall v^{n+1} \in \mathbb U_h,
	 \\[0.5cm]
b( u^{n+1},  q^{n+1} ) = 0 & \forall q^{n+1} \in \mathbb Q_h,
\end{cases}
\end{equation}
where, for the sake of clarity, we remark that 
$$
a_s(u^{n+1};u^{n+1},v^{n+1}) =  \int_{\Omega} \nu_T(\overline{\Pi}_h u^{n+1})\nabla \overline{\Pi}_h u^{n+1} : \nabla \overline{\Pi}_h v^{n+1} \; dx.
$$
with the following expression for the Eddy viscosity 
\begin{equation}
    \label{eq:eddy_nu}
    \nu_T(\overline{\Pi}_h u^{n+1}) = c_s^2 \sum_{K \in \mathcal T} h_k^2 |\nabla (\overline{\Pi}_h u^{n+1})|\chi_K, 
\end{equation}
\label{sec:FE}
with $| \cdot |$ denoting the Frobenius norm in $\mathbb R^{d \times d}$, $\chi_K$ the characteristic function over a triangle $K$ and $c_s$ Smagorinsky's constant \ms{cite}. 



==> sections/VSMSMEF.tex <==
\section{VMS-Smagorinsky Evolve-Filter\ti{Correct?} Algorithm}
\label{sec:VMSSMEF}
In this section we propose a new regularized algorithm to deal with convection dominated NSE.\\
The idea is to apply standard filtering techniques \ms{cite} only to the resolved small scales of the velocity field.
\ms{add some more intro}

\subsection{The linear strategy} 
Convection-dominated flows %may 
{generally} lead to spurious numerical oscillations when the spatial resolution is larger than the Kolomogorov lengthscale, which inversely proportional to the Reynolds number~\cite{Fri95,Pop00}.
\begin{eqnarray}
         &	\text{(I)}& \text{\emph{ Evolve}:} \quad 
\begin{cases}
        	  \displaystyle \int_{\Omega} \frac{w^{n+1} - u^{n}}{\Delta t}\cdot v^{n+1}_h \; dx & \\
	\quad \quad\quad\quad \quad\quad\quad + a(w^{n+1},  v^{n+1})
	 & \\ \quad \quad\quad\quad \quad \quad\quad
 \quad \quad \quad+ c(w^{n+1}; w^{n+1}, v^{n+1})
  & \\ 
  \quad \quad\quad\quad \quad\quad \quad \quad\quad\quad \quad\quad \quad \quad  - b(v^{n+1}, p^{n+1}) &  \forall v^{n+1} \in \mathbb U_h,
	 \\[0.5cm]
b( w^{n+1},  q^{n+1} ) = 0 & \forall q^{n+1} \in \mathbb Q_h,
\end{cases}
            \label{eqn:ef-rom-1}\nonumber \\[0.3cm]
            &	\text{(II)} &\text{\emph{ Filter:}} \quad
\begin{cases} \nonumber
        	 \displaystyle \delta^2 \int_{\Omega} \nabla \overline{w}^{n+1} : \nabla v^{n+1} \; dx +  \int_{\Omega} \overline{w}^{n+1} v^{n+1} \; dx  = \int_{\Omega}{{w}'^{n+1}} v^{n+1} & \forall v^{n+1} \in \mathbb U_h, \vspace{1mm}\\
\overline{w}^{n+1} = u^{n+1}_D &\text{on } \Gamma_D , \vspace{1mm}\\
\displaystyle \frac{\partial \overline{w}^{n+1}}{\partial  n} = 0  & \text{on } \Gamma_N .
\end{cases}
	\nonumber \\[0.3cm]
            &	\text{(III)} &\text{\emph{\ms{name?} \ti{Correct?}}} \qquad 
        	   u^{n+1} = \widetilde{w}^{n+1} + \overline{w}^{n+1}.
            \nonumber
\end{eqnarray}

{In step (I), we evolve an input velocity $u^n$ to an intermediate velocity $\widetilde{u}^{n+1}$ by standard VMS-Smagorinsky model for time $t^{n+1}$.
In step (II), we apply a \emph{differential filter} (DF) 
of filtering radius $\delta$ the intermediate velocity approximation, $\widetilde{u}^{n+1}$, obtained in step (I).
The action of the DF is to alleviate oscillations by means of an elliptic operator that eliminates the high frequencies that might arise in the resolved small-scales of the flow. Last, in step (III) we relax the filtered intermediate velocity at time $t^{n+1}$ to increase the accuracy of the simulation by a convex combination between $\widetilde{w}^{n+1}$ and $\overline{w}^{n+1}$ for $\chi \in (0,1)$ \ms{cite stuff}.




\subsection{The nonlinear Strategy} \ms{some more intro and maybe I write it down in strong form}
\begin{eqnarray}
         &	\text{(I)}& \text{\emph{ Evolve}:} \quad 
\begin{cases}
        	  \displaystyle \int_{\Omega} \frac{w^{n+1} - u^{n}}{\Delta t}\cdot v^{n+1}_h \; dx & \\
	\quad \quad\quad\quad \quad\quad\quad + a(w^{n+1},  v^{n+1})
	 & \\ \quad \quad\quad\quad \quad \quad\quad
 \quad \quad \quad+ c(w^{n+1}; w^{n+1}, v^{n+1})
  & \\ 
  \quad \quad\quad\quad \quad\quad \quad \quad\quad\quad \quad\quad \quad \quad  - b(v^{n+1}, p^{n+1}) & \forall v^{n+1} \in \mathbb U_h,
	 \\[0.5cm]
b( w^{n+1},  q^{n+1} ) = 0 & \forall q^{n+1} \in \mathbb Q_h,
\end{cases}
            \nonumber \\[0.3cm]
            &	\text{(II)} &\text{\emph{ Filter:}} \quad
\begin{cases} \nonumber
        	 \displaystyle \nu_T(w'^{n+1}) \int_{\Omega} \nabla \overline{w}^{n+1} : \nabla v^{n+1} \; dx +  \int_{\Omega} \overline{w}^{n+1} v^{n+1} \; dx  = \int_{\Omega}{{w'}^{n+1}} v^{n+1} & \forall v^{n+1} \in \mathbb U_h, \vspace{1mm}\\
\overline{w}^{n+1} = u^{n+1}_D &\text{on } \Gamma_D , \vspace{1mm}\\
\displaystyle \frac{\partial \overline{w}^{n+1}}{\partial  n} = 0  & \text{on } \Gamma_N .
\end{cases}
	 \nonumber \\[0.3cm]
            &	\text{(III)} &\text{\emph{\ms{name?} \ti{Correct?}}} \qquad 
        	   u^{n+1} = \widetilde{w}^{n+1} + \overline{w}^{n+1}.
            \nonumber
\end{eqnarray}

{In step (I), we evolve an input velocity $u^n$ to an intermediate velocity %$\widetilde{u}^{n+1}$ 
\ti{$w^{n+1}$} by standard VMS-Smagorinsky model for time $t^{n+1}$.
In step (II), we apply a \emph{differential filter} (DF) 
of filtering radius $\delta$ to filter only the resolved small-scale velocity $w'^{n+1} = \overline{\Pi_h}w^{n+1}$ of the intermediate velocity approximation, $\widetilde{u}^{n+1}$, obtained in step (I).
The action of the DF is to alleviate oscillations by means of an elliptic operator that eliminates the high frequencies that might arise in the resolved small-scales of the flow. Last, in step (III) we define the filtered input at time $t^{n+1}$ as the sum of resolved large scales of $w^{n+1}$, i.e.\ $\widetilde{w}^{n+1}$ and the filtered resolved small-scales  $\overline{w}^{n+1}$.
}

\subsection{The alternative strategy} \ms{some more intro and maybe I write it down in strong form}

\begin{eqnarray}
         &	\text{(I)}& \text{\emph{ Evolve}:} \quad 
\begin{cases}
        	  \displaystyle \int_{\Omega} \frac{w^{n+1} - u^{n}}{\Delta t}\cdot v^{n+1}_h \; dx & \\
	\quad \quad\quad\quad \quad\quad\quad + a(w^{n+1},  v^{n+1})
	 & \\ \quad \quad\quad\quad \quad \quad\quad
 \quad \quad \quad+ c(w^{n+1}; w^{n+1}, v^{n+1})
  & \\ 
  \quad \quad\quad\quad \quad\quad \quad \quad\quad\quad \quad\quad \quad \quad  - b(v^{n+1}, p^{n+1}) & \forall v^{n+1} \in \mathbb U_h,
	 \\[0.5cm]
b( w^{n+1},  q^{n+1} ) = 0 & \forall q^{n+1} \in \mathbb Q_h,
\end{cases}
            \nonumber \\[0.3cm]
            &	\text{(II)} &\text{\emph{ Filter over $w^{n+1}$:}} \quad
\begin{cases} \nonumber
        	 \displaystyle C \int_{\Omega} \nabla \overline{w}^{n+1} : \nabla v^{n+1} \; dx +  \int_{\Omega} \overline{w}^{n+1} v^{n+1} \; dx  = \int_{\Omega}{{w}^{n+1}} v^{n+1} & \forall v^{n+1} \in \mathbb U_h, \vspace{1mm}\\
\overline{w}^{n+1} = u^{n+1}_D &\text{on } \Gamma_D , \vspace{1mm}\\
\displaystyle \frac{\partial \overline{w}^{n+1}}{\partial  n} = 0  & \text{on } \Gamma_N .
\end{cases}
	 \nonumber \\[0.3cm]
              &	\text{(II)} &\text{\emph{ Filter over $\widetilde{w}^{n+1}$}} \quad
\begin{cases} \nonumber
        	 \displaystyle C \int_{\Omega} \nabla \overline{\widetilde{w}}^{n+1} : \nabla v^{n+1} \; dx +  \int_{\Omega} \overline{\widetilde{w}}^{n+1} v^{n+1} \; dx  = \int_{\Omega}{\widetilde{w}^{n+1}} v^{n+1} & \forall v^{n+1} \in \widetilde{\mathbb U}_h, \vspace{1mm}\\
\overline{\widetilde{w}}^{n+1} = u^{n+1}_D &\text{on } \Gamma_D , \vspace{1mm}\\
\displaystyle \frac{\partial \overline{\widetilde{w}}^{n+1}}{\partial  n} = 0  & \text{on } \Gamma_N .
\end{cases}
	 \nonumber \\[0.3cm]
            &	\text{(III)} &\text{\emph{\ms{name?} \ti{Correct?}}} \qquad 
        	   u^{n+1} = \widetilde{w}^{n+1} + (\overline{w}^{n+1} - \overline{\widetilde{w}}^{n+1}).
            \nonumber
\end{eqnarray}

